A Hardware-Aware Gate Cutting Framework for Practical Quantum Circuit Knitting

Circuit knitting emerges as a promising technique to overcome the limitation of the few physical qubits in near-term quantum hardware by cutting large quantum circuits into smaller subcircuits. Recent research in this area has been primarily oriented towards reducing subcircuit sampling overhead. Unfortunately, these works neglect hardware information during circuit cutting, thus posing significant challenges to the follow on stages. In fact, direct compilation and execution of these partitioned subcircuits yields low-fidelity results, highlighting the need for a more holistic optimization strategy. In this work, we propose a hardware-aware framework aiming to advance the practicability of circuit knitting. Drawing a contrast with prior methodologies, the presented framework designs a cutting scheme that concurrently optimizes the number of gate cuttings and SWAP insertions during circuit cutting. In particular, we leverage the graph similarity between qubits interactions and chip layout as a heuristic guide to reduces potential SWAPs in the subsequent step of qubit routing. Building upon this, the circuit knitting framework we developed has been evaluated on several quantum algorithms, leading to reduction of total subcircuits depth by up to 64% (48% on average) compared to the state-of-the-art approach, and enhancing the relative fidelity up to 2.7$\times$.

==> fig_kronecker.tex <==
\usepackage{graphicx}
\usepackage{svg}
\usepackage{subcaption}
\usepackage{tikz}
\usepackage[export]{adjustbox}
\usepackage{pdfpages}
\usepackage{textcomp}
\usepackage{xcolor}
\def\BibTeX{{\rm B\kern-.05em{\sc i\kern-.025em b}\kern-.08em
    T\kern-.1667em\lower.7ex\hbox{E}\kern-.125emX}}
\newcommand{\myz}[1]{{\color{blue}{#1}}}
\newcommand{\todo}[1]{{\color{red}{#1}}}
\usepackage{ulem}
\usepackage{qcircuit}

\definecolor{light_purple}{RGB}{188,189,220}
\begin{figure*}[ht]
\centering
\begin{minipage}[]{.2\textwidth}
    \Qcircuit @C=1.2em @R=.8em {
    & \qw & \qwa  &&&   \gate{Z} &  \qwa & & & & \displaystyle\sum_{\alpha_1 = \pm 1} \alpha_1 & & & \meterB{{}_{=\alpha_1}}           & \qwa & & & & \displaystyle\sum_{\alpha_1 = \pm 1} \alpha_1 & & & \gate{R_Z(\frac{\alpha_1\pi}{2})} & \qwa \\ 
    & \otimes & & + & & \otimes & &         + & & & & & & \otimes & &                                                                           + & & & & & & \otimes \\
    & \qw & \qwa  &&&   \gate{Z} &  \qwa & & & & \displaystyle\sum_{\alpha_2 = \pm 1} \alpha_2 & & & \gate{R_Z(\frac{\alpha_2\pi}{2})} & \qwa & & & & \displaystyle\sum_{\alpha_2 = \pm 1} \alpha_2 & & & \meterB{{}_{=\alpha_2}} & \qwa 
    \gategroup{1}{1}{1}{3}{.7em}{.} \gategroup{1}{5}{1}{7}{1.5em}{.} \gategroup{1}{10}{1}{15}{2.8em}{.} \gategroup{1}{18}{1}{23}{2.8em}{.}
    \gategroup{3}{1}{3}{3}{.7em}{.} \gategroup{3}{5}{3}{7}{1.5em}{.} \gategroup{3}{10}{3}{15}{2.8em}{.} \gategroup{3}{18}{3}{23}{2.8em}{.}
    }
\end{minipage}
\hfill
\begin{minipage}[]{.2\textwidth}
    \begin{tikzpicture}
        \node[draw,shape=circle,scale=1.6,fill=light_purple] (v0) at (0,-0.1) {};
        \node[draw,shape=circle,scale=1.6,fill=light_purple] (v1) at (0,-2.1){};
        \draw [line width=3pt]  (v0) -- (0.6,-0.1) (1,-0.1)   node {$2^{q_1}$}
                                (v1) -- (0.6,-2.1) (1,-2.1) node {$2^{q_2}$};
        \draw [thick]   (v0) -- (0,-0.65) (0,-1.55) -- (v1) 
                        (-1.3,-1.1) node {$\rightarrow$}
                        (0,-0.85) node {$4$} (0,-1.35) node {$4$};
    \end{tikzpicture}
\end{minipage}
\caption{Classical Postprocessing with Kronecker Product}
\label{fig:kronecker}
\end{figure*}

==> spacetrick.tex <==
% -*- root: main.tex -*-

%space left between floats.
\setlength{\floatsep}{2mm}
% space between last top float or first bottom float and the text.
\setlength{\textfloatsep}{2mm}

% space left on top and bottom of an in-text float.
\setlength{\intextsep}{0.5mm}
% space above caption
\setlength{\abovecaptionskip}{2mm}
%space below caption
\setlength{\belowcaptionskip}{0mm}

%% Change figure handling
\renewcommand{\topfraction}{0.9}
\renewcommand{\textfraction}{0.1}
\renewcommand{\floatpagefraction}{1}

\usepackage[small,compact,noindentafter]{titlesec}
% \usepackage[compact]{titlesec}

\titlespacing\section{0pt}{6pt plus 2pt minus 2pt}{2pt plus 2pt minus 2pt}
\titlespacing\subsection{0pt}{4pt plus 2pt minus 2pt}{2pt plus 1pt minus 1pt}
\titlespacing\subsubsection{0pt}{2pt plus 0pt minus 1pt}{1.0ex}
\titlespacing{\paragraph}{0pt}{2pt plus 0pt minus 1pt}{1.0ex}

\usepackage[inline]{enumitem}
\setlist{noitemsep,topsep=0pt,parsep=0pt,partopsep=0pt}

\usepackage[subtle]{savetrees}
% \usepackage[moderate]{savetrees}

\usepackage{setspace}
\usepackage[margin=0pt,skip=0pt,font={stretch=0.9}]{caption}
\usepackage[margin=5pt,font={stretch=0.9}]{caption}
\usepackage[margin=8pt,font={small,bf,stretch=0.85}]{caption}

% \titleformat{\subsection}
%  {\normalfont\fontsize{12}{15}\bfseries}{\thesection}{1em}{}


